A Note on Reachability and Distance Oracles for Transmission Graphs

Let $P$ be a set of $n$ points in the plane, where each point $p\in P$ has a transmission radius $r(p)>0$. The transmission graph defined by $P$ and the given radii, denoted by $\mathcal{G}_{\mathrm{tr}}(P)$, is the directed graph whose nodes are the points in $P$ and that contains the arcs $(p,q)$ such that $|pq|\leq r(p)$. An and Oh [Algorithmica 2022] presented a reachability oracle for transmission graphs. Their oracle uses $O(n^{5/3})$ storage and, given two query points $s,t\in P$, can decide in $O(n^{2/3})$ time if there is a path from $s$ to $t$ in $\mathcal{G}_{\mathrm{tr}}(P)$. We show that the clique-based separators introduced by De Berg \emph{et al.} [SICOMP 2020] can be used to improve the storage of the oracle to $O(n\sqrt{n})$ and the query time to $O(\sqrt{n})$. Our oracle can be extended to approximate distance queries: we can construct, for a given parameter $\varepsilon>0$, an oracle that uses $O((n/\varepsilon)\sqrt{n}\log n)$ storage and that can report in $O((\sqrt{n}/\varepsilon)\log n)$ time a value $d_{\mathrm{hop}}^*(s,t)$ satisfying $d_{\mathrm{hop}}(s,t) \leq d_{\mathrm{hop}}^*(s,t) < (1+\varepsilon)\cdot d_{\mathrm{hop}}(s,t) + 1$, where $d_{\mathrm{hop}}(s,t)$ is the hop-distance from $s$ to $t$. We also show how to extend the oracle to so-called continuous queries, where the target point $t$ can be any point in the plane. To obtain an efficient preprocessing algorithm, we show that a clique-based separator of a set~$F$ of convex fat objects in $\Bbb{R}^d$ can be constructed in $O(n\log n)$ time.

==> extensions.tex <==
%------------------------------------------------------------------------------------------
\section{Extensions}
\label{sec:extensions}
%------------------------------------------------------------------------------------------
